Reconstruction of Neutrino-Induced Hadronic and Electromagnetic Showers with the ANTARES Experiment

The ANTARES neutrino telescope is being constructed at a site off the French Mediterranean coast at a depth of 2400m. When high energy neutrinos interact in water, the charged secondary particles produce Cherenkov light which can be measured in photomultiplier tubes. Different event signatures are possible; this work introduces a reconstruction algorithm for events with a hadronic and potentially an electromagnetic shower producing a signal in the detector. An algorithm for the combined reconstruction of shower direction and energy is described, based on a maximum likelihood fit which matches the signal expected in the photomultipliers for an assumed direction and energy with the signal actually measured.

==> q.tex <==
\relax 
\@setckpt{Theory/background}{
\setcounter{page}{4}
\setcounter{equation}{0}
\setcounter{enumi}{0}
\setcounter{enumii}{0}
\setcounter{enumiii}{0}
\setcounter{enumiv}{0}
\setcounter{footnote}{2}
\setcounter{mpfootnote}{0}
\setcounter{part}{0}
\setcounter{chapter}{1}
\setcounter{section}{0}
\setcounter{subsection}{0}
\setcounter{subsubsection}{0}
\setcounter{paragraph}{0}
\setcounter{subparagraph}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{parentequation}{0}
}

